Isotropic atomic layer etching of MgO-doped lithium niobate using sequential exposures of H$_2$ and SF$_6$ plasmas

Lithium niobate (LiNbO$_3$, LN) is a ferroelectric crystal of interest for integrated photonics owing to its large second-order optical nonlinearity and the ability to impart periodic poling via an external electric field. However, on-chip device performance based on thin-film lithium niobate (TFLN) is presently limited by propagation losses arising from surface roughness and corrugations. Atomic layer etching (ALE) could potentially smooth these features and thereby increase photonic performance, but no ALE process has been reported for LN. Here, we report an isotropic ALE process for $x$-cut MgO-doped LN using sequential exposures of H$_2$ and SF$_6$/Ar plasmas. We observe an etch rate of $1.59 \pm 0.02$ nm/cycle with a synergy of $96.9$%. We also demonstrate ALE can be achieved with SF$_6$/O$_2$ or Cl$_2$/BCl$_3$ plasma exposures in place of the SF$_6$/Ar plasma step with synergies of $99.5$% and $91.5$% respectively. The process is found to decrease the sidewall surface roughness of TFLN waveguides etched by physical Ar$^+$ milling by 30% without additional wet processing. Our ALE process could be used to smooth sidewall surfaces of TFLN waveguides as a post-processing treatment, thereby increasing the performance of TFLN nanophotonic devices and enabling new integrated photonic device capabilities.

==> scratch.tex <==
% and ultimately enabling novel devices not attainable in other integrated photonic platforms

% , which is similar to four cationic layer distances for bulk LN,

 % compared to other photonic materials like SiN

 
% induced by Ar$^+$ milling and the difference in etching rate of regions of oppposite poling
% The introduction of thin-film lithium niobate (TFLN) based on ion-slicing has enabled photonic circuits with improved figures of merit on account of the greater refractive index contrast than is achievable in bulk LN.

% and saturation of etch rates with respect of plasma exposure time

 % owing to its ability to smooth surfaces to sub-nanometer length scales
% , the standard technique used for nanophotonic LN waveguide fabrication. Further, the etch depth control achievable with Ar$^+$ milling is around $\pm 20$ nanometers,  directly impacting the dispersion and ideal quasi-phase matching poling period of the circuits.

% In addition to pure Ar+ milling, the most widely adopted means of transferring patterns to this platform, often leads to large etch depth variations which
% Ryoto's intro:
% From fiber-optic communications to photonic quantum technologies [link], lithium niobate (LiNbO3 or LN) has been a mainstay for many photonic applications. A ferroelectric crystal with a large electro-optic bandwidth, UV-MIR transparency window, and most importantly a high second-order nonlinear susceptibility, LN allows for a plethora of nonlinear optical phenomena unavailable in other common photonic platforms such as silicon nitride (SiN). Early efforts with bulk LN include weakly confining waveguides, usually based on Ti ion diffusion or proton exchanged LN. 
% With the advent of smart-cut, thin-films of lithium niobate (TFLN) have become commercially available. The tighter mode confinement as well as the increased freedom to engineer the dispersion and quasi-phase-matching (QPM) properties of propagating light have enabled nanophotonic circuits demonstrating record on-chip quantum states, 500 GHz electro-optic modulators with CMOS compatible voltages (Phase Sensitive Inc.), and multi-octave frequency comb sources with fJ-level pump pulse energies.
% Despite these impressive demonstrations, the current method of fabricating these nanophotonic TFLN circuits imposes severe limitations in terms of platform scalability and increased performance. Pure Ar+ milling, the most widely adopted means of transferring patterns to this platform, often leads to large etch depth variations which directly impact the dispersion and ideal QPM poling period of the circuits. In addition, the Ar+ milling process leaves enough side wall roughness such that the material limited Q-factor for TFLN waveguides is estimated to be an order of magnitude away from current waveguides. 
% These challenges could be addressed by ALE …..
% It is worth noting that previous attempts at using fluorine and chlorine based RIE lead to  … redeposition suffer. But ALE can get around it!

% , which does not have electro-optic or nonlinear-optic properties in a similarly wide transparency window

% limits etch depth

%**also try to quantify, perhaps using the figure from the proposal


% In the device community, physical Ar$^+$ milling remains the preferred dry etch method used for pattern transfer. However, this method has its own limitations such as low etch selectivity with common lithography resists and non-vertical sidewalls. \cite{Zhu:21, Ar_LN_Etch_Clean} Additionally, etch depth tolerances for photonic devices are desired to be $\sim \pm$5 nm to operate in a regime near the desired group-velocity dispersion (GVD) and group-velocity mismatch (GVM) values, \cite{Ledezma_etchdepth, Jankowski_etchdepth} a tolerance which is difficult to achieve with Ar$^+$ milling.  As a result, various device figures of merit are far from their intrinsic upper limits. For instance, the material-limited quality factor for TFLN micro-ring resonators is estimated to be an order of magnitude higher than that realized in present devices due to losses from surface roughness scattering. \cite{Kippenberg_Loncar_MaterialQ} Decreasing losses and increasing etch depth precision in TFLN circuits will enable system-level integration of on-chip nonlinear optics and allow for quantum information processing. \cite{Zhu:21}

% These issues are difficult to deal with in periodically-poled LN (PPLN).


% For instance, the dominant loss mechanism TFLN devices come from scattering losses in corrugations in PPLN . 

% ***to avoid any unintended issues with submission, pls move commented text to scratch.tex file
% We now discuss the characteristics of our directional LN ALE process in context with other pattern transfer processes for LN. Ar$^+$ milling etch rates are linear with time, while RIE processes suffer from the redeposition of nonvolatile lithium compounds such as LiF. The present recipe is able to achieve nanometer-level EPC. The self-limiting nature of both half-steps of the process enables the etch depth precision and reduces the variation in etch rates between different chamber processing conditions.

% **let's narrow the scope, the process as it is cannot yield precise etch depths due to F redeposition. that can be moved to future work. this process can be used for corrugation loss and roughness loss. some ref should be cited (find ref from proposal) showing that corrugation loss is dominant

% This process has the potential to serve as a post-processing step to achieve improved etch depth precision within several nanometers of the target value. The use of this process as post-processing step will therefore allow the desired GVM and GVD to be achieved, in turn enabling improved device characteristics such as a larger phase-matching bandwidth or higher efficiency of nonlinear frequency conversion. 

%****what does effective mean? you mean ALE processes have been developed which etch metal oxides?




%------------SIMS Results--------------------------
% SIMS analysis was performed using a Cameca IMS 7f-GEO secondary-ion mass spectrometer using a Cesium ion beam at 2 nA ion beam current. Prior to analysis, samples were sputter coated in 10 nm of gold to reduce charging effects. The estimated depth for each point was calculated by using AFM to determine the total sputtered depth and 
% assuming a constant ion sputtering rate. The relative H and Li content between the samples is determined by normalizing the hydrogen counts by the O$^-$ content of the films.



 % Although the ALE process increases surface roughness due to LiF and MgF$_2$ redeposition, we show that the surface can be smoothened with a subsequent RCA clean.

 

% Achieving such etch depth accuracy in TFLN will 
% ALE of LN may increase the performance of existing TFLN devices and enable novel devices not attainable in other integrated photonic platforms.

% $x$-cut LN has a cationic interatomic distance of $0.23$ nm at the surface and $0.26$ nm in the bulk crystal. \cite{sanna_linbo3_2017} For simplicity, we consider the bulk interatomic distance and this EPC corresponds to 

%is similar to****similar to is too fuzzy, make a quantitative comparison and think what is the claim you are making by including this statement


% *****keep a uniform tense, before this is past, and next phrase is present tense. usually in results we use present tense throughout. pls check throughout as I may not catch everything.

%In comparison, the SF$_6$/Ar process with identical plasma exposure times had an etch rate of $0.XX \pm 0.XX$  nm/cycle over 20 cycles with a synergy of XX\%. 

% **I think some subsections could be helpful


% **I think first figure should be present 4d. we need it more zoomed in? it is definitely true that this feature could not be produced by an isotropic process? If we are not sure, due to tight time, perhaps leave off directional in the claim for now and sort it out later?

%Frank's comment:  I suggest you plot the figure as nm vs. nm to zoom in on the slope and the microtrenching.
% My response: I feel like zooming in very close will take away from the message of the figure, which is that the etch is directional. It would be confusing because it would look like a linear slope
%***AJM: Can you paste his suggested plot in slack?




% After Ar$^+$ milling, the redeposited LN is removed with HF or RCA, which introduces  corrugations in PPLN. Our ALE process can be used to reduce the corrugation step heights and an alternate wet etch will 


% ***may need to mention another method for removing redeposited product is needed to avoid recreating the corrugations

% surface roughness losses, achieving precise etch depths across the entire chip, and smoothing corrugations in periodically-poled LN (PPLN). Ar milling typically produces sidewall angles of $\sim 40-80 \degree$ \cite{Zhu:21}, and the deviation from perfectly vertical sidewalls limits the minimum feature size and distance between structures. Additionally, sputtered LN is redeposited onto the film,  necessitating a follow-up wet cleanup step using HF or RCA etchant which introduces corrugations in PPLN. The present process could be used after Ar$^+$ milling to smooth the micron-sized corrugation features in PPLN.

% Further, the nominal poling period for quasi-phase-matching critically depends on the waveguide geometry such as top width, etch depth, and the total LN film thickness.\cite{sekine2023multioctave} The present process could be used after Ar$^+$ milling to obtain etch depths within the desired group-velocity mismatch and group-velocity dispersion regimes.

% The uncertainty in etch depth is governed by the increase in surface roughness from Li and Mg redeposition as the number of ALE cycles increase. In addition, the increase in roughness during ALE can be mitigated with an RCA clean. The ALE system in our work (Oxford Instruments, Plasma Pro 100 Cobra) is able to process 200 mm diameter substrates, and therefore our process has the potential to extend to wafer-scale applications.

% the cycle count due to the 

% **try to focus this para, it is now a list of interesting future topics but a bit lacking in coherency. for instance, one organizing theme could be the redeposition issue and the different ways to address it, e.g. gas-based removal, Cl plasma, etc

%****same issue here regarding RCA clean. also the ALE process by itself does not have potential to smooth sidewalls.



% .  % This ability is expected to enable improved TFLN device performance and potential functionalities which are not achievable in other integrated photonics platforms.

% With this, TFLN devices can be reliably etched to the target etch depth required for the desired GVM and GVD.

% From AFM and XPS analysis, we conclude that LiF redeposition occurs over cycle numbers, causing surface roughness that can be removed with a subsequent RCA clean.


% and that it can be mitigated using the standard procedure already in use for TFLN device fabrication. However, 


% Similarly to Ar$^+$ milled TFLN, the increase in roughness can be improved with a wet etch. After 

% , indicating that the H$_2$ plasma exposure is not reducing surface Li concentration and producing proton-exchanged LN in contrast with in Fig. 4 in Ref.~\cite{Ren_PE_LN_Plasma}, where an hour-long H$_2$ plasma exposure produced proton-exchanged LN.

% ***extra context and some citation is needed, you could even refer to the specific figure number with SIMS

%(x to y percent, or is this qualitative) Qualitative, quantitative analysis in next para looking at the atomic conc.

%********so do these alternate recipes yield multiples of cationic distance? if not, what is significance compared to the added statements before? 
% they do not yield multiples of cationic distance, but they are also not at saturation probably.
%due to the uncertainty, almost any EPC could be considered to be a multiple of the EPC? I am not sure these statements provide much insight


% We note that this EPC corresponds to four cationic layer distances.



%These alternate reported recipes are not saturated at the given plasma exposure times, and as a result EPC does not yield multiples of cationic layer distance.
%***I still feel like the reason why these statements are made is never stated anywhere

% . Further, we report that SF$_6$/Ar plasma can be replaced with either an O$_2$/SF$_6$ or Cl$_2$/BCl$_3$ plasma to achieve ALE with synergies exceeding 90\% in both cases and find that the Cl$_2$/BCl$_3$ process produces the least surface roughness increase following ALE. 

% These observations sets the stage for further investigation of the use of ALE process in the fabrication of LN integrated photonic devices.

%***in this para, describe at a high level the key findings of the paper

% Despite the extensive desirable optical properties of LN, the development of LN photonic devices is limited by the methods of fabrication. The presence of lithium in lithium niobate presents limitations in the fabrication of LN nanophotonic devices due to the redeposition of lithium compound redeposition. We developed a recipe specifically for X-cut MgO-doped lithium niobate, which is the material of choice used for integrated photonics due to the raised optical damage threshold and polarizability compared to lithium niobate. This development provides a new, more precise way for plasma etching of this material, and with different etch chemistries which are compatible with different etch masks. We expect that these findings can be used to advance the state of the art in LN photonic device development, and that this development will be of interest to the readers of JVSTA.
